ClassEval: A Manually-Crafted Benchmark for Evaluating LLMs on Class-level Code Generation

In this work, we make the first attempt to evaluate LLMs in a more challenging code generation scenario, i.e. class-level code generation. We first manually construct the first class-level code generation benchmark ClassEval of 100 class-level Python code generation tasks with approximately 500 person-hours. Based on it, we then perform the first study of 11 state-of-the-art LLMs on class-level code generation. Based on our results, we have the following main findings. First, we find that all existing LLMs show much worse performance on class-level code generation compared to on standalone method-level code generation benchmarks like HumanEval; and the method-level coding ability cannot equivalently reflect the class-level coding ability among LLMs. Second, we find that GPT-4 and GPT-3.5 still exhibit dominate superior than other LLMs on class-level code generation, and the second-tier models includes Instruct-Starcoder, Instruct-Codegen, and Wizardcoder with very similar performance. Third, we find that generating the entire class all at once (i.e. holistic generation strategy) is the best generation strategy only for GPT-4 and GPT-3.5, while method-by-method generation (i.e. incremental and compositional) is better strategies for the other models with limited ability of understanding long instructions and utilizing the middle information. Lastly, we find the limited model ability of generating method-dependent code and discuss the frequent error types in generated classes. Our benchmark is available at https://github.com/FudanSELab/ClassEval.

==> sections/evaluation/composition_generation.tex <==
\individualgen generation pertains to the process in which each method is independently crafted before being consolidated to formulate the final comprehensive class. This technique can be viewed as a progressive extension of the method-level generation concept.

More specifily, the primary objective of generation is to construct class-level code by individually generating each method and subsequently integrating these distinct components into a cohesive unit to form the complete class-level code.
Throughout the generation of each method, apart from furnishing the correspond method contract design, the process also incorporates vital dependency information necessary for the method. This could entail the inclusion of import statements (if applicable), along with the class constructor and the signatures of other methods within the class (a requisite).

\textbf{IF LLMs.}
The design of the given prompt aligns with the strategy employed during the Incremental Generation experiments as delineated in Section \ref{sec:incremental_generation}.
Nevertheless, it diverges from the incremental generation paradigm in a fundamental way: rather than incorporating the previously generated method body into the successive input, each method generated for this particular task only contains its specific method contract design, import statements, as well as class initialization and other method signatures within the class. In an endeavor to obviate possible misinterpretations and to narrow the focus of LLMs on the specific method, we have incorporated a "Pass" code snippet succeeding all other method signatures. This modification ensures that LLMs prioritize the generation of the target method, without the burden of completing other method signatures.
\textbf{FIM LLMs.}

\textbf{NTP LLMs.}
NTP LLMs share the same input format as FIM LLMs.

==> sections/evaluation/holistic_generation.tex <==
\holisticgen{} generation assesses the LLMs' capability to comprehend class skeletons and process extensive textual information for simultaneous code generation. It requires LLMs to possess a comprehensive understanding of the overall structure and requirements associated with class-level code generation tasks.

\textbf{IF LLMs.} For LLMs that can follow instructions, we design a prompt representing the instructions to ask them to complete the class based on the class skeleton. The template is shown below:

\begin{mdframed}[linecolor=white!50,linewidth=2pt,roundcorner=10pt,backgroundcolor=myyellow!20]
\noindent \{ \textbf{System Prompt} \}

\noindent \#\#\# Instruction:

\noindent \{ \textbf{Instruction} \}

\noindent \#\#\# Response:
\end{mdframed}
\lmw{describe what is the system prompt and what if for}
The \textit{system prompt} in the template serves as the initial sentence in the prompt \textcolor{red}{to xxxx} and is typically defined by each LLM individually.
To identify the most effective and comprehensive \textit{system prompt}, we conducted extensive experimentation and selected the optimal \textit{system prompt} as follows:
\lmw{describe why our system prompt look like this, can we say we refer/adapt it from some existing paper? we need to describe where are the initial seed system prompts from?}
\begin{mdframed}
[linecolor=white!50,linewidth=2pt,roundcorner=10pt,backgroundcolor=myyellow!20]
\noindent \textbf{System Prompt:} Provided below is an instruction detailing a task. Compose a response that aptly fulfills the request.
\end{mdframed}

Additionally, the \textit{Instruction} in the template provides a detailed task description for LLMs to accomplish. The \textit{instruction} for \holisticgen{} (\textit{Instruction-H}) is formulated as follows, where {Class Name} and {Class Skeleton} need to be replaced with the specific task information: \lmw{say how do we get the instruction} 

\begin{mdframed}
[linecolor=white!50,linewidth=2pt,roundcorner=10pt,backgroundcolor=myyellow!20]
\noindent \textbf{Instruction-1:} Please complete the class \{Class Name\} in the subsequent code. \{Class Skeleton\}
\end{mdframed}

\begin{mdframed}
[linecolor=white!50,linewidth=2pt,roundcorner=10pt,backgroundcolor=myyellow!20]
\textbf{Instruction-2:} Please complete the method \{ method name \} within the following class \{ class name \}. \{ Class Context \}
\end{mdframed}


\textbf{FIM LLMs:} For FIM LLMs, we convert the class-level code generation task into an infilling task. We provide the complete class skeleton as input, with the addition of \textit{<insert>} tags following each method contract design. These tags serve as hints for FIM LLMs to generate the corresponding code at the specific location within the class skeleton.


\textbf{NTP LLMs:} For NTP LLMs, we use the class skeleton as direct input and instruct the models to continue generating the text.











==> sections/evaluation/incremental_generation.tex <==
The \incrementalgen{} generation involves generating each method sequentially, using contextual information from the preceding methods to build the complete class. This iterative process reflects the progressive nature of software development, where developers incrementally build upon existing code to achieve the final desired functionality of the class.

In detail, the generation entails an iterative process commencing with the initial input of the class description, class name, class constructor, as well as the signature and description of the first target method. Following the successful generation of the first method's code, this output is amalgamated with the aforementioned input, further augmented by the inclusion of the signature and description pertaining to the second method. This iterative mechanism of step by step code generation perpetuates until the completion of code generation for all the methods within the class. 
% \lmw{define docstring? or use other term}
Throughout the entire iterative process, crucial class-level contextual information, termed as the \textit{Class Context}, is provided to LLMs at each step. Figure \ref{fig:incremental_generation} provides a graphical representation of the Class Context's evolution through each iterative step of the generation process.

\textbf{IF LLMs.} For IF LLMs, the prompt employed for generating each method is crafted following the guidelines set forth in Section~\ref{sec:holistic_generation}, albeit with a modification to the instruction as follows:
\begin{mdframed}
[linecolor=white!50,linewidth=2pt,roundcorner=10pt,backgroundcolor=myyellow!20]
\textbf{Instruction:} Please complete the method \{ method name \} within the following class \{ class name \}. \{ Class Context \}
\end{mdframed}

\textbf{FIM LLMs.}
For FIM LLMs, the class context is directly used as input for each iteration. In this case, the generation process follows a similar iterative approach, with the class context being provided as input to the model for each iteration. 

\textbf{NTP LLMs.} 
NTP LLMs share the same input format as FIM LLMs.

During the \incrementalgen{} generation process, we enforce a method generation order that fulfills the following condition: when a method exhibits method dependencies, we prioritize generating the dependent methods before their corresponding calling methods. By adhering to this method generation order, we effectively avoid any potential problems related to ungenerated method dependencies

==> tables/evaluation.tex <==

\begin{table*}[htp]
    \scriptsize	
 %\footnotesize
	\centering
    \vspace{-4mm}
	\caption{Prompts for Three Class-level Code Generation Strategies}
	\label{table:gen_input}
	\vspace{-2mm}
        \begin{adjustbox}{width=2.1\columnwidth}
	\begin{tabular}{c|ccc}
		\hline
		\textbf{Strategy} & \textbf{LLM Type} & \textbf{Prompt with Context Information} & \textbf{Output} \\ \hline
        \multirow{3}{*}{\tabincell{c}{\holisticgen{} \\ Generation}}
    	 & IF  &  System Prompt + Instruction-1 + Class Skeleton & Class  \\ \cline{2-4} 
    	& FIM & Class Skeleton with <insert> Tags  & Methods  \\ \cline{2-4} 
            & NTP & Class Skeleton  & Class  \\ \hline
        \multirow{2}{*}{\tabincell{c}{\incrementalgen{}\\ Generation}}
    	 & IF  & {System Prompt} + Instruction-2 + Class-level Info + Generated Methods with Contract Designs + Target Method Contract Design & Method \\ \cline{2-4} 
            & FIM/NTP& Class-level Info + Generated Methods with Contract Designs + Target Method Contract Design  & Method \\ \hline
        \multirow{2}{*}{\tabincell{c}{\individualgen{}\\ Generation }}
    	 & IF  & {System Prompt} + Instruction-3 + Class-level Info + Other Method Signatures + Target Method Contract Design  & Method  \\ \cline{2-4} 
           & FIM/NTP & Class-level Info + Other Method Signatures + Target Method Contract Design & Method  \\ \hline
	\end{tabular}
        \end{adjustbox}
	% \vspace{-7.5mm}
\end{table*}



